Satisfying Real-world Goals with Dataset Constraints

The goal of minimizing misclassification error on a training set is often just one of several real-world goals that might be defined on different datasets. For example, one may require a classifier to also make positive predictions at some specified rate for some subpopulation (fairness), or to achieve a specified empirical recall. Other real-world goals include reducing churn with respect to a previously deployed model, or stabilizing online training. In this paper we propose handling multiple goals on multiple datasets by training with dataset constraints, using the ramp penalty to accurately quantify costs, and present an efficient algorithm to approximately optimize the resulting non-convex constrained optimization problem. Experiments on both benchmark and real-world industry datasets demonstrate the effectiveness of our approach.

==> Makefile <==
LATEX = latex
PDFLATEX = pdflatex -file-line-error -halt-on-error
PS2PDF = ps2pdf

SPELLCHECK_FILES = $(wildcard main.tex abstract.tex sec-*.tex app-*.tex figures/*.tex theorems/*.tex)
TEX_FILES = $(wildcard *.tex */*.tex)
EPS_IMAGES = $(wildcard images/eps/*.eps)
PDF_IMAGES = $(wildcard images/pdf/*.pdf)
FILES = $(TEX_FILES) $(EPS_IMAGES) $(PDF_IMAGES)

BEGIN_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:begin}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'
MIDDLE_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:middle}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'
APPENDIX_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:appendix}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'
END_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:end}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'

.PHONY : all
all: main.pdf main.bbl

%.bbl: %.bib $(FILES)
	$(MAKE) -C images
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}
	bibtex ${basename $<}

%.pdf: %.tex %.bbl $(FILES)
	$(MAKE) -C images
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}

dictionary.txt: words.txt main.bib $(SPELLCHECK_FILES)
	cp words.txt dictionary.txt
	cat main.bib | sed -n "s/^@[^{]*{//p" | sed "s/,[[:space:]]*$$//" | sed "s/[[:punct:][:digit:]].*$$//" | sort | uniq >> dictionary.txt
	#cat $(SPELLCHECK_FILES) | sed -n "s/^.*\\label{\([^}]*\)}.*$$/\1/p" | sed "s/[:-]/\n/g" | sort | uniq >> dictionary.txt

dictionary.rws: dictionary.txt
	aspell --lang=en create master ./$@ < $<

spellcheck: dictionary.rws $(SPELLCHECK_FILES)
	for ii in $(SPELLCHECK_FILES) ; do aspell -d en_US --extra-dicts=`pwd`/dictionary.rws -c $$ii ; done

.PHONY: clean
clean:
	$(MAKE) -C images clean
	rm -f dictionary.txt dictionary.rws
	rm -f main.log main.aux main.bbl main.blg main.out
	rm -f main.pdf main.bbl


==> figures/fig-churn-small.tex <==
\begin{figure*}[t]

\begin{center}

\begin{tabularx}{\textwidth}{cc}
  %
  \includegraphics[width=\plotwidth]{images/churn_vs_churn_target} &
  %
  \includegraphics[width=\plotwidth]{images/error_vs_churn_target}
  %
\end{tabularx}

\end{center}

\caption{
  %
  Blue: our proposal, with the classification functions' predictions being
  deterministically thresholded at zero.
  %
  Red: same, but using the randomized classification rule described in
  \secref{problem}.
  %
  Green: unconstrained SVM trained on $D_1 \cup D_2$, then thresholded (by
  shifting the bias $b$) to satisfy the recall constraint on $D_2$.
  %
  Dashed and dotted curves denote results on the testing and training datasets,
  respectively.
  %
  \textbf{(Left)} Observed churn (vertical axis) vs. the churn target used
  during training (horizontal axis), on the unlabeled dataset $D_3$.
  %
  \textbf{(Right)} Empirical error rates (vertical axis) vs. the churn target,
  on the union $D_1 \cup D_2$ of the two labeled datasets.
  %
  All curves are averaged over 10 runs.
  %
}

\label{fig:churn}

\end{figure*}


==> figures/fig-ramp-bounds-small.tex <==
\begin{wrapfigure}{r}{\plotwidth}

\vspace{-4em}

\begin{center}

\includegraphics[width=\plotwidth]{images/ramp_bounds}

\end{center}

\caption{
  %
  Convex upper bounds on the ramp function $\sigma(z)=\max\left\{ 0,\min\left\{
  1,\nicefrac{1}{2}+z\right\} \right\}$. Notice that the hinge bound (red) is
  tight for all $z\le\nicefrac{1}{2}$, and the constant bound (blue) is tight
  for all $z\ge\nicefrac{1}{2}$.
  %
}

\label{fig:ramp-bounds}

\end{wrapfigure}

